The De Broglie-Bohm theory {\it is} and {\it is not} a hidden variable theory

We will first define what is meant by ``hidden variables". Then, we will review various theorems proving the impossibility of theories introducing such variables and then show that the de Broglie-Bohm theory is not refuted by those theorems. We will also explain the relation between those theorems and nonlocality, with or without introducing Bell's inequalities.

==> option_keys.tex <==
\ifx\optionkeymacros\undefined\else\endinput\fi
% This document is in the Public Domain.
% It was created by Doug Henderson, Blue Sky Research,
% with modifications suggested by Joseph C. V‡rilly.
% Added single quotes on 6-4-93.
%
% option_keys - 6-4-93 (last modification)
%
% This macro set defines characters found in the Apple Macintosh
% Monaco font. They allow users to simply type the keystroke 
% equivalent of the character desired, such as ¿, and have Texturesª
% typeset it correctly, substituting the TeX macro equivalent
% for the character.
%
% The reason for the creation of this macro set was to take 
% advantage of Knuth's new TeX 3.0 capabilities with 8-bit character
% sets. This functionality has been included in our Texturesª as
% of version 1.3. By typing in nearly any character from the 
% Macintosh keyboard, you can typeset with the characters directly 
% rather than needing to define macros for these diacritic characters. 
% Remember: these just expand single characters. They may not be
% defined in every context or mode.
%
% There are two sections to the macros; the first contains
% characters which can be rendered by depressing the option key
% and another key or shift and option keys with another key, 
% and secondly, a combination of various keystrokes together 
% to obtain the desired character. For example,
% to create the ¿ character, you depress the option and o character
% at the same time; to create the uppercase version of ¯, you 
% hold the shift, option key, and o key down, and to create the
% " character, you first depress the option and n characters, 
% then next the shift and n characters. The option and n create
% the tilde character, and the shift n produce the N character.
%
% Math symbols and math operators need special attention. 
% When typing in math symbols the same 
% rules apply for math mode as before, namely, you must place dollar
% signs or double-dollar signs around these symbols. When typing
% in math operators, such as the square root symbol, TeX expects
% you to supply an argument following it. For example, if you
% would like to take advantage of the definition here for the
% plus-minus sign, ±, and would like to type it directly for use
% in your text, you need to make sure you are in math mode when
% you call for the character, or simply place dollar signs around
% it to print only the plus minus sign thusly, $±$. Similarly,
% you also need to be in math mode when asking for the square root
% symbol, Ã, and additionally supply an argument to it. 
% The following example shows how to use both the plus-minus sign
% and the square root sign in an equation that has been simplified
% for you via these macro definitions.
%      $$-b±Ã{b^2-4ac}\over{2a}$$

% define the macintosh "option" generated characters

\catcode`\Œ=\active\defŒ{{\aa}}       % option a
\catcode`\º=\active\defº{\int}        % option b (math mode) 
\catcode`\=\active\def{\c c}        % option c
\catcode`\¶=\active\def¶{\partial}    % option d (math mode)
\catcode`\Ä=\active\defÄ{\oint}       % option f (math mode) ?
\catcode`\Æ=\active\defÆ{\triangle}   % option j (math mode)
\catcode`\Â=\active\defÂ{\neg}        % option l (math mode)
\catcode`\µ=\active\defµ{\mu}         % option m (math mode)
\catcode`\¿=\active\def¿{{\o}}        % option o
\catcode`\¹=\active\def¹{\pi}         % option p (math mode w/ arg.)
\catcode`\Ï=\active\defÏ{{\oe}}       % option q 
\catcode`\§=\active\def§{{\ss}}       % option s 
\catcode`\ =\active\def {\dagger}     % option t  (math mode)
\catcode`\Ã=\active\defÃ{\sqrt}       % option v (math mode w/ arg.)
\catcode`\·=\active\def·{\Sigma}      % option w (math mode)
\catcode`\Å=\active\defÅ{\approx}     % option x (math mode)
\catcode`\½=\active\def½{\Omega}      % option z (math mode)
\catcode`\£=\active\def£{{\it\$}}     % option 3 ($ from italic font)
\catcode`\°=\active\def°{\infty}      % option 5 (math mode)
\catcode`\¤=\active\def¤{{\S}}        % option 6 
\catcode`\¦=\active\def¦{{\P}}        % option 7
\catcode`\¥=\active\def¥{\bullet}     % option 8 
\catcode`\»=\active\def»{\leavevmode\raise.585ex\hbox{\b a}}      % option 9
\catcode`\¼=\active\def¼{\leavevmode\raise.6ex\hbox{\b o}}        % option 0
\catcode`\­=\active\def­{\not=}       % option = (math mode)
\catcode`\²=\active\def²{\leq}        % option , (math mode)
\catcode`\³=\active\def³{\geq}        % option . (math mode)
\catcode`\Ö=\active\defÖ{\div}        % option / (math mode)
\catcode`\É=\active\defÉ{{\dots}}     % option ; 
\catcode`\¾=\active\def¾{{\ae}}       % option '
\catcode`\Ç=\active\defÇ{\ll}         % option \ (math mode)
\catcode`\Ò=\active\defÒ{``}          % option [
\catcode`\Á=\active\defÁ{!`}          % option !
\catcode`\¢=\active\def¢{\rlap/c}     % option 4
\catcode`\Ô=\active\defÔ{`}           % option ] 
\catcode`\Õ=\active\defÕ{'}           % shift option ]

% macintosh "shift-option" generated characters

\catcode`\=\active\def{{\AA}}       % shift-option A
\catcode`\'=\active\def'{\c C}        % shift-option C
\catcode`\¯=\active\def¯{{\O}}        % shift-option O
\catcode`\¸=\active\def¸{\Pi}         % shift-option P (math mode)
\catcode`\Î=\active\defÎ{{\OE}}       % shift-option Q
\catcode`\®=\active\def®{{\AE}}       % shift-option '
\catcode`\×=\active\def×{\diamond}    % shift-option V (math mode)
\catcode`\¡=\active\def¡{\accent'27}  % shift-option 8
\catcode`\Ó=\active\defÓ{''}          % shift-option [
\catcode`\±=\active\def±{\pm}         % shift-option = (math mode)
\catcode`\È=\active\defÈ{\gg}         % shift-option \ (math mode)
\catcode`\À=\active\defÀ{?`}          % shift-option / 
\catcode`\Ð=\active\defÐ{--}          % option - (en-dash)
\catcode`\Ñ=\active\defÑ{---}         % shift-option - (em-dash)

% define the macintosh "composite" characters

\catcode`\Š=\active\defŠ{\"a}        % option u, then  a
\catcode`\'=\active\def'{\"e}        % option u, then  e
\catcode`\•=\active\def•{\"{\i}}     % option u, then  i
\catcode`\š=\active\defš{\"o}        % option u, then  o
\catcode`\Ÿ=\active\defŸ{\"u}        % option u, then  u
\catcode`\Ø=\active\defØ{\"y}        % option u, then  y
\catcode`\€=\active\def€{\"A}        % option u, then  A
\catcode`\…=\active\def…{\"O}        % option u, then  O
\catcode`\†=\active\def†{\"U}        % option u, then  U
\catcode`\‡=\active\def‡{\'a}        % option e, then  a
\catcode`\Ž=\active\defŽ{\'e}        % option e, then  e
\catcode`\'=\active\def'{\'{\i}}     % option e, then  i
\catcode`\—=\active\def—{\'o}        % option e, then  o
\catcode`\œ=\active\defœ{\'u}        % option e, then  u
\catcode`\ƒ=\active\defƒ{\'E}        % option e, then  E
\catcode`\ˆ=\active\defˆ{\`a}        % option `, then  a
\catcode`\=\active\def{\`e}        % option `, then  e
\catcode`\"=\active\def"{\`{\i}}     % option `, then  i
\catcode`\˜=\active\def˜{\`o}        % option `, then  o
\catcode`\=\active\def{\`u}        % option `, then  u
\catcode`\Ë=\active\defË{\`A}        % option `, then  A
\catcode`\‹=\active\def‹{\~a}        % option n, then  a
\catcode`\–=\active\def–{\~n}        % option n, then  n
\catcode`\›=\active\def›{\~o}        % option n, then  o
\catcode`\Ì=\active\defÌ{\~A}        % option n, then  A
\catcode`\"=\active\def"{\~N}        % option n, then  N
\catcode`\Í=\active\defÍ{\~O}        % option n, then  O
\catcode`\‰=\active\def‰{\^a}        % option i, then  a
\catcode`\=\active\def{\^e}        % option i, then  e
\catcode`\"=\active\def"{\^{\i}}     % option i, then  i
\catcode`\™=\active\def™{\^o}        % option i, then  o
\catcode`\ž=\active\defž{\^u}        % option i, then  u

\let\optionkeymacros\null

